iDPA: Instance Decoupled Prompt Attention for Incremental Medical Object Detection

Existing prompt-based approaches have demonstrated impressive performance in continual learning, leveraging pre-trained large-scale models for classification tasks; however, the tight coupling between foreground-background information and the coupled attention between prompts and image-text tokens present significant challenges in incremental medical object detection tasks, due to the conceptual gap between medical and natural domains. To overcome these challenges, we introduce the \method~framework, which comprises two main components: 1) Instance-level Prompt Generation (\ipg), which decouples fine-grained instance-level knowledge from images and generates prompts that focus on dense predictions, and 2) Decoupled Prompt Attention (\dpa), which decouples the original prompt attention, enabling a more direct and efficient transfer of prompt information while reducing memory usage and mitigating catastrophic forgetting. We collect 13 clinical, cross-modal, multi-organ, and multi-category datasets, referred to as \dataset, and experiments demonstrate that \method~outperforms existing SOTA methods, with FAP improvements of 5.44\%, 4.83\%, 12.88\%, and 4.59\% in full data, 1-shot, 10-shot, and 50-shot settings, respectively.

==> tables/exp_encoder.tex <==
\begin{table}[t]
  \centering
      \caption{Number of $\theta_{\text{inc}}$-inserted encoder analysis. 
      }
     
      \label{table:ablation_L}
      \small
      \setlength{\tabcolsep}{2.5pt} %
    \fontsize{13pt}{15pt}\selectfont
     \renewcommand{\arraystretch}{4.0}%
  

   { \fontsize{8.3}{3}\selectfont{
      \begin{tabular}{ccc|*{3}c|cc}
     \toprule
      $\Phi_{\bf v}$&$\Phi_{\bf t}$&$\Phi_{\bf f}$&$\text{FAP} \uparrow$  &$\text{AAP}\downarrow$&${\text{FPP}}\uparrow$ &\#Params $\downarrow$ &\#Memory $\downarrow$\\
       \midrule
          \cmark &\xmark& \xmark & 44.4 & 56.8 & 45.4  & 12k  & 12k  \\
          \xmark &\cmark& \xmark  & 47.3 & 57.5 & 48.1  & 53K & 53K \\
          \cmark &\cmark& \xmark  & 49.0 & 58.2 & 49.7 & 94K & 94K \\
          \xmark &\xmark& \cmark   & 50.1 & 59.9 & 50.8 & 135K& 135K  \\
          \cmark &\cmark& \cmark   & 51.3 & 59.7 & 51.9 & 258K & 258K \\
      \bottomrule
      \end{tabular}
      }}
      \vspace{-0.5em}
\end{table}


==> tables/exp_scale.tex <==
\begin{table}[t]
  \centering
      \caption{Performance gap between {\method} and {\method} with oracle retrieval module.}
      \label{table:ablation_retrieval}
      \small
      \setlength{\tabcolsep}{6pt} %
     \renewcommand{\arraystretch}{4.0}%
   { \fontsize{8.3}{3}\selectfont{
      \begin{tabular}{c|ccccc}
      \bottomrule
      Scale&$\text{FAP}$&$\text{FAP}^{\text{50}}$&$\text{FAP}^{\text{75}}$&$\text{AAP}$  &$\text{FPP}$\\
       \hline      
      Constant (1.0)  &45.55	&73.28	&48.98	&49.99	&2.61 \\
      Gate  &44.65	&72.59	&47.53	&50.29	&1.18 \\
      Dim-wise  &46.61	& &		&51.30	&3.95  \\
      Ours (task-wise)  &47.86	&76.53	&50.90	&52.06	&2.47 \\
      \toprule
      \end{tabular}
      }}
      \vspace{-2em}
  \end{table}

==> tables/exp_seq.tex <==
\begin{table}[t]
  \centering
      \caption{Performance gap between {\method} and {\method} with oracle retrieval module.}
      \label{table:ablation_retrieval}
      \small
      \setlength{\tabcolsep}{6pt} %
     \renewcommand{\arraystretch}{4.0}%
   { \fontsize{8.3}{3}\selectfont{
      \begin{tabular}{c|ccccc}
      \bottomrule
      Context&$\text{FAP}$&$\text{FAP}^{\text{50}}$&$\text{FAP}^{\text{75}}$&$\text{AAP}$  &$\text{FPP}$\\
       \hline
        
      Gaussian Noise  &&&&& \\
      Images  &&&&& \\
      Instances  &&&&&  \\
      \toprule
      \end{tabular}
      }}
      \vspace{-2em}
  \end{table}
